Distributed transactional reads: the strong, the quick, the fresh \& the impossible

This paper studies the costs and trade-offs of providing transactional consistent reads in a distributed storage system. We identify the following dimensions: read consistency, read delay (latency), and data freshness. We show that there is a three-way trade-off between them, which can be summarised as follows: (i) it is not possible to ensure at the same time order-preserving (e.g., causally-consistent) or atomic reads, Minimal Delay, and maximal freshness; thus, reading data that is the most fresh without delay is possible only in a weakly-isolated mode; (ii) to ensure atomic or order-preserving reads at Minimal Delay imposes to read data from the past (not fresh); (iii) however, order-preserving minimal-delay reads can be fresher than atomic; (iv) reading atomic or order-preserving data at maximal freshness may block reads or writes indefinitely. Our impossibility results hold independently of other features of the database, such as update semantics (totally ordered or not) or data model (structured or unstructured). Guided by these results, we modify an existing protocol to ensure minimal-delay reads (at the cost of freshness) under atomic-visibility and causally-consistent semantics. Our experimental evaluation supports the theoretical results.

==> Makefile <==
# Important commands:
#	make update	# download repository version and merge
#	make commit	# upload to repository
#	make		# generate pdf
#	make bib	# generate bibliogrphy
#	make force	# generate bibliogrphy and force re-run
#	make clean	# remove temp files
#	make spotless   # idem + remove pdf, bib files

# Please do not add .pdf or other generated files to SVN targets.  Thanks!

FILE=middleware18-authorversion

MAKEFLAGS=	--no-print-directory

# ------------------------------
# User configurable dependencies
# ------------------------------

# GNUPlot source files
GPSOURCE= \
	$(wildcard figures/*.gp)

# EPS files included
EPSSOURCE= \
	$(wildcard figures/*.eps)

# PDF files included
PDFSOURCE= \
	related-wor2.pdf \
	figures/3-way-tradeoff.pdf

# PNG files included
PNG= 

	# $(wildcard figures/*.png)

# BIB files included
BIBS= \
	references1.bib \
	predef.bib \
	shapiro-bib-ext.bib \
	shapiro-bib-perso.bib

# local.bib

# Bibtex style
BST= \
	abbrvnat-no-url.bst

# .tex file includes or inputs
#	abstract-v2-ale.tex \

TEXIN= ${TXT} ${SRC}

TXT= \
	abstract.tex \
	introduction.tex \
	model.tex \
	tradeoff.tex \
	protocols.tex \
	evaluation.tex \
	related-work.tex \
	conclusion.tex

SRC= 
# \
     # 	tm-pseudocode.tex \
     # 	p-pseudocode.tex \
     # 	s-pseudocode.tex 

# other file dependencies
DEPS= Makefile

# files that are not Make dependencies but are required nonetheless
OTHERCOMMITS= \
	figures/3-way-tradeoff.key \
	related-wor2.numbers

MANUAL= \
	figures/3-way-tradeoff.pdf \
	related-wor2.pdf


#
# MANUAL: add the following after default:
#
# figures/fig.png: figures/figures.key
# 	@echo "Must first recreate $@ from $<!!" 2>&1
# 	@false

# ------------------------------
# End user configurable dependencies
# ------------------------------

EPSGEN=$(GPSOURCE:.gp=.eps)
EPSGRAPHICS= ${EPSGEN} ${EPSSOURCE}

PDFGEN=$(EPSGRAPHICS:.eps=.pdf)
PDFGRAPHICS=${PDFGEN} ${PDFSOURCE}

GRAPHICSSOURCE= ${GPSOURCE} ${EPSSOURCE} ${PDFSOURCE} ${PNG}
GRAPHICSGEN=${EPSGEN} ${PDFGEN}

TEXTDEPS=${FILE}.tex ${TEXIN} ${DEPS}
GRAPHICDEPS= ${PDFGRAPHICS} ${PNG}

SOURCES= ${EPSSOURCE}  ${GPSOURCE}  ${EPSSOURCE}  ${PDFSOURCE}  ${PNG}  ${BIBS}  ${TEXIN} ${BST}
ALLFILES= ${FILE}.tex ${SOURCES} ${DEPS} ${OTHERCOMMITS}

GNUPLOT= gnuplot 

# ------------------------------
# source control
# ------------------------------
default: etags pdf

txt:
	open ${TXT} ${FILE}.tex

figures/3-way-tradeoff.png: figures/3-way-tradeoff.key
	@echo "Must first recreate $@ from $<!!" 2>&1
	@false

related-wor2.pdf: related-wor2.numbers
	@echo "Must first recreate $@ from $<!!" 2>&1
	@false

pull update:
	svn update
#	git pull

push commit: ${MANUAL}
	-svn propset svn:keywords 'URL Date Revision Author' ${FILE}.tex
# unset LANG because it influences the way SVN generates the date inside the file
# explicit ${ALLFILES} to verify that they have all been declared by 'svn add'
	unset LANG; svn commit -m '' ${ALLFILES}
	# git add ${ALLFILES}
	# git commit --allow-empty --allow-empty-message -m ""
	# git push origin master
# also commit files not in dependencies
	unset LANG; svn commit -m ''
	# git add -u
	# git commit --allow-empty --allow-empty-message -m ""
	# git push origin master

spotless:: clean

# begin diff
# requires latexdiff from http://www.ctan.org/tex-archive/support/latexdiff/
diff: $(FILE)-diff.pdf

remotebase svnbase:
	svn cat $(FILE).tex > $(FILE)-base.tex

localbase base savebase:
	cp $(FILE).tex $(FILE)-base.tex

$(FILE)-diff.tex: $(FILE)-base.tex $(FILE).tex
	latexdiff $(FILE)-base.tex $(FILE).tex > $(FILE)-diff.tex

$(FILE)-diff.aux: $(FILE).aux
	cp $(FILE).aux $(FILE)-diff.aux

$(FILE)-diff.bbl: $(FILE).bbl
	cp $(FILE).bbl $(FILE)-diff.bbl

$(FILE)-diff.pdf: $(FILE)-diff.tex $(FILE)-diff.aux $(FILE)-diff.bbl
	pdflatex $(FILE)-diff.tex

clean::
	-rm -f $(FILE)-diff.* $(FILE)-base.*

# end diff

# ---------- latex compilation ----------

tags etags: TAGS

TAGS: ${TEXTDEPS}
	etags ${TEXTDEPS}

clean::
	rm -f TAGS

graphics: epsgraphics pdfgraphics

epsgraphics: ${EPSGRAPHICS}

pdfgraphics: ${PDFGRAPHICS}

# dvi: $(FILE).dvi 

show: pdf
	open $(FILE).pdf

pdf: $(FILE).pdf

print lpr: $(FILE).pdf
	lpr $(FILE).pdf

# $(FILE).dvi: $(FILE).tex $(FIGS)

aux: $(FILE).aux

$(FILE).pdf ${FILE}.aux: ${TEXTDEPS} ${GRAPHICDEPS}
	pdflatex $(FILE)

### $(FILE).dvi ${FILE}.aux: ${FILE}.tex ${DEPS} ${EPSGRAPHICS} ${PNG}
### 	latex $(FILE)

#figs:
#		( cd figs; $(MAKE) )
clean::
		/bin/rm -f *~ *.bak *.aux *.log *.toc *.lof *.dvi *.bbl *.blg *.lot *.out
		/bin/rm -rf auto/

spotless:: 
		/bin/rm -f ${FILE}.pdf

# ---------- bibliography ----------

force: bib forcepdf1 default forcepdf2

forcepdf1 forcepdf2: FORCE
	pdflatex $(FILE)

FORCE:

${FILE}.bbl: aux ${BST} ${BIBS} 
		-bibtex ${FILE}
#		./bibnourl.sh ${BIBS}
#		BIBINPUTS=tmp/:$$BIBINPUTS bibtex $(FILE)
#		sed -e 's/%//g' < $(FILE).bbl > $(FILE).bbl~
#		mv $(FILE).bbl~ $(FILE).bbl

# clean::
# 	rm -rf tmp/

bib: $(FILE).bbl 

# effective only for user @shapiro
ifeq ($(shell whoami),shapiro)
shapiro-bib-ext.bib: /Users/shapiro/svnbackup/bib/shapiro-bib-ext.bib
	cp -p /Users/shapiro/svnbackup/bib/shapiro-bib-ext.bib .

shapiro-bib-perso.bib: /Users/shapiro/svnbackup/bib/shapiro-bib-perso.bib
	cp -p /Users/shapiro/svnbackup/bib/shapiro-bib-perso.bib .

predef.bib: /Users/shapiro/svnbackup/bib/predef.bib
	cp -p /Users/shapiro/svnbackup/bib/predef.bib .

short-predef.bib: /Users/shapiro/svnbackup/bib/short-predef.bib
	cp -p /Users/shapiro/svnbackup/bib/short-predef.bib .

grassroots.bib: /nobackup/svnstuff/syncfree_SVN/papers/grassroots.bib
	ln -s /nobackup/svnstuff/syncfree_SVN/papers/grassroots.bib .

spotless::
	rm -f shapiro-bib-perso.bib shapiro-bib-ext.bib predef.bib short-predef.bib grassroots.bib
endif
# end only @shapiro

# ---------- html ----------

html: ${FILE}.html

${FILE}.html ${FILE}.css: ${FILE}/${FILE}.html
	cp -p ${FILE}/${FILE}.html .
	cp -p ${FILE}/${FILE}.css .

${FILE}/${FILE}.html: ${FILE}.aux
	latex2html -split 0 ${FILE}

clean::
	rm -rf ${FILE}/

spotless::
	rm -f ${FILE}.html ${FILE}.css

# ---------- standard targets ----------

%.eps: %.obj
	tgif -print -eps $^
%.eps: %.gp
	$(GNUPLOT) $^

# %.eps: %.gp dat/%.dat
#	$(GNUPLOT) $^

%.eps: %.fig
	fig2dev -L eps $^ >$@
%.eps: %.prn
	ps2epsi $^ $@
clean::
	rm -f ${GRAPHICSGEN}

%.eps: %.dia
	dia -e $@ $^
%.eps: %.epsraw
	ps2epsi $^ $@

%.pdf: %.tex
	pdflatex $^

%.bbl: %.aux
	-bibtex $^

# According to ACM instructions, '-P cmz' embeds Type 1 fonts, which
# enables later PDF generation to be of higher quality 
# %.ps: %.dvi
# 	dvips -P cmz $^ -o
# 	rm -f $@.gz

%.pdf: %.ps
	ps2pdf $^
%.pdf: %.eps
	epstopdf $^

tgz: ${FILE}.pdf
	dir=`basename $$PWD`; \
	tar czvf /tmp/$(FILE).tgz -C .. \
	$(patsubst %,$$dir/%,\
	    ${ALLFILES} \
	    ${patsubst %,dat/%,${GPSOURCE:.gp=.dat}}\
	)

zip: ${FILE}.pdf
	rm -rf /tmp/$(FILE).zip; \
	zip /tmp/$(FILE).zip \
	    ${ALLFILES} \
	    ${patsubst %,dat/%,${GPSOURCE:.gp=.dat}}




==> future-work.tex <==
\chapter{Unexplored Isolation Levels}
\label{chap:new-isolation}


% \begin{table}
% \centering
% %   \hspace*{-1em}
%   \begin{tabular}{>{\centering}m{7cm} | c | c  }
%    \textbf{Isolation Level} & \textbf{Snapshot guarantees} & \textbf{Reads follow Writes} \\
%    \hline
%    Strict Serialisability (SS) & Atomic Visibility & Monotonically \\
%    Serialisability (S) & Atomic Visibility & Monotonically \\
%    Update Serialisability (US) & Atomic Visibility & Non Monotonically \\
%    Snapshot Isolation (SI) & Atomic Visibility & Monotonically \\
%    Parallel Snapshot Isolation (PSI) & Atomic Visibility & Non Monotonically \\
%    Transactional Causal Consistency (TCC) & Atomic Visibility & Non Monotonically \\
%    Read Atomic  (RA) & Atomic Visibility & Non Monotonically \\
%    Read Committed (RC) & Committed Visibility  & Monotonically \\
% \end{tabular}
% \caption{Read properties of existing isolation levels}
% \label{table:read-isolation}
% \end{table}


% \begin{table}
% \centering
% %   \hspace*{-1em}
%   \begin{tabular}{>{\centering}m{3.5cm} | >{\centering}m{2.5cm} | >{\centering}m{2cm} | c | c }
%    \textbf{Isolation Level} & \textbf{Serial. Checks} & \textbf{Snapshot} & \textbf{Update order} & \textbf{Snapshot order} \\
%    \hline
%    Strict Serialisability (SS) & Reads and Writes & Atomic Visibility & Monotonic & Monotonic \\
%    Serialisability (S) & Reads and Writes & Atomic Visibility  & Monotonic & Monotonic \\
%    Update Serialisability (US) & Reads and Writes(*) & Atomic Visibility  & Monotonic & Non Monotonic \\
%    Snapshot Isolation (SI) & Writes & Atomic Visibility  & Monotonic & Monotonic \\
%    Parallel Snapshot Isolation (PSI) & Writes & Atomic Visibility  & Non Monotonic & Non Monotonic \\
%    \textbf{PSI--} & \textbf{Writes} & \textbf{OP Visibility}  & \textbf{Non Monotonic} & \textbf{Non Monotonic} \\
%    Transactional Causal Consistency (TCC) & None & Atomic Visibility  & Non Monotonic & Non Monotonic \\
%    \textbf{TCC--} & \textbf{None} & \textbf{OP Visibility}  &\textbf{ Non Monotonic }& \textbf{Non Monotonic} \\
%    Read Atomic  (RA) & None  & Atomic Visibility  & Non Monotonic & Non Monotonic \\
%    Read Committed (RC) & None  & Committed Visibility   & Non Monotonic & Non Monotonic \\
% \end{tabular}
% \caption{Properties of existing isolation levels}
% \label{table:isolation-guarantees}
% \end{table}






An isolation level restricts the interleaving of the operations
of one transaction with those of others, in order
to forbid certain anomalous behaviours.
Under multi-version concurrency control,
a transaction reads from a snapshot.  
When committing, a commit protocol checks that the 
operations of the transaction have interleaved with
the operations of other transactions only in ways permitted
by the isolation level it implements (Section \ref{sec:mvcc}).
In Section \ref{sec-apguarantees}, we
discussed the three snapshot
guarantees considered for the trade-off.
In this chapter, we discuss some new 
isolation levels that result from the
combinations of those snapshot properties with different
commit guarantees.
Table \ref{table:update-isolation} shows the properties of the combinations
of read and commit guarantees.
Order-Preserving Visibility can be combined in unexplored ways.
\textbf{TCC--} is the combination of Order-Preserving Visibility with 
non-serialised atomic updates.
\textbf{PSI--} combines Order-Preserving Visibility
with write serialisation (or write-write conflict) checks. 
Changing Update Serialisability (US) so that 
read-only transactions ensure Committed and Order-Preserving visibility results in
two models, which we call \textbf{CV-US} and \textbf{OP-US}, respectively.
% \footnote{We do not discuss these two models, as their update transactions remain identical
% to those of US. The differences of reads have been discussed in Chapters \ref{sec-apguarantees}
% and \ref{sec-tradeoff}.}
Table \ref{table:anomalies2} compares the anomalies of several models.



\begin{table}
\centering
\small
%   \hspace*{-1em}
  \begin{tabular}{ >{\centering}m{3.8cm} | c | c | c | c | c |c}
    \multirow{4}{*}{\textbf{Snapshot / Termination}} & \multicolumn{4}{c|}{\textbf{Non-monotonic Order}} 	& \multicolumn{2}{c}{\textbf{Monotonic Order}} \\
    												& \multicolumn{4}{c|}{\textbf{of Operations}} & \multicolumn{2}{c}{\textbf{of Operations}} \\
   \cline{2-7}
    & \textbf{Not} & \multicolumn{2}{c|}{\textbf{Ser.}}  & \textbf{Ser.} & \textbf{Ser.} & \textbf{Ser.} \\
    & \textbf{Ser.} & \multicolumn{2}{c|}{\textbf{Writes}} & \textbf{R. and W.} & \textbf{Writes}  & \textbf{R. and W.} \\
   \Xhline{3\arrayrulewidth}
   Committed  		& RC			 & \multicolumn{2}{c|}{RC+}	 		   & \textit{\textbf{CV-US}}  & \multirow{2}{*}{N/A} & \multirow{2}{*}{N/A} \\
   \cline{1-5}
   Order-Preserving		& \textit{\textbf{TCC--}}	 & \multicolumn{2}{c|}{\textit{\textbf{PSI--}}}  & \textit{\textbf{OP-US}} & & \\
   \hline
   Atomic  			& TCC$\slash$RA	 & \multicolumn{2}{c|}{PSI} 	   & US & SI & S \\

  \end{tabular}
  \caption{Combination of snapshot and termination guarantees - In bold: combinations not previously studied}
\label{table:update-isolation}
\end{table}
%
%
%
% \bigskip\noindent\textbf{Non-considered read$\slash$termination combinations.}
% Table \ref{table:update-isolation} distinguishes the snapshot guarantees,
% ordering of operations (monotonic or non monotonic) and serialisation checks
% of several models.
% Some combinations are not considered (and not shown in the table):
%
% \begin{compactitem}
% \item\textbf{Non-monotonic updates and serialisable (read and update) operations.}
% Serialisation creates a monotonic total order of operations.
% This combination is not possible.
%
% \item\textbf{Monotonic updates without serialisation}
% are not considered, as they normally expose states that is
% temporarily incorrect.
% For instance, it is possible to generate a total order of
% updates by allowing concurrent updates, and later resolve
% them using a Last-Write-Wins policy.
% However, this
%
%
% \item\textbf{Monotonic Reads and Non-Monotonic Updates.}
% Monotonic snapshots are possible when updates follow a total order.
% Observing a monotonic total order of snapshots consisting of non-monotonically-ordered
% updates is a contradiction.
% \end{compactitem}

% \section{New isolation properties}
%
% We introduce the properties of unexplored isolation levels.
% Table \ref{table:anomalies2} shows the anomaly comparison of these models and existing ones.

\section{CV-US and OP-US}
Under Update Serialisability (US), only update transactions are serialisable.
Read-only transactions read from Atomically-consistent snapshots that do not form
a monotonic order.
CV-US relaxes the guarantees of read-only transactions
to Committed Visibility and, OP-US, from relaxing reads to Order-Preserving visibility.
% We do not further elaborate on the semantics of these two models, as the modifications
% they make over Update Serialisability only affect read-only transactions, and a comparison
% of read guarantees has been introduced in Section \ref{sec-apguarantees}.


\section{TCC--}
\label{sec:tcc-}

Under Transactional Causal Consistency (TCC), a transaction reads from an atomically-consistent snapshot.
Both reads and updates can be concurrent (they are not serialised).
TCC-- weakens TCC's read guarantees to Order-Preserving Visibility.
Therefore, when compared to TCC, TCC-- further allows the read-skew anomaly.
On the positive side, as the results of the trade-off show, this relaxation positions TCC-- in a better
position with respect to latency and freshness.
In the next chapter, we introduce a protocol offering these guarantees.
In Section \ref{sec-evaluation}, we evaluate this protocol in terms of latency, throughput, and freshness.


\section{PSI--}
\label{sec:psi-}

Under Parallel Snapshot Isolation (PSI), a transaction reads from an atomically-consistent snapshot,
and updates are serialised.
PSI-- weakens the read guarantees to Order-Preserving Visibility.
Compared to PSI, PSI-- adds the read-skew anomaly.
In line with our study of trade-offs,
this relaxation can improve the latency and freshness of PSI--.

Fresh reads have the potential to reduce the abort rate of update transactions. 
An implementation of PSI requires reading up-to-date data to commit a transaction.
When committing, it must verify that other transactions
do not update the same objects concurrently.
For each object updated, if there exists an update since
the transaction's snapshot, the transaction aborts.

An interesting observation is that under a similar implementation,
a protocol ensuring PSI-- disallows Read Skews over the objects
a transaction updates.
This occurs because serialisation disallows the existence of versions
more up-to date than those read by the transaction. 
An experienced programmer desiring the latency/freshness properties of Order-Preserving reads
could issue updates on the particular objects it requires reading atomically.
Unfortunately, we have not experimented with algorithms implementing PSI--.
% Nevertheless, as we will see in the our evaluation (Section \ref{sec-evaluation}),
% freshness results suggest that the reduction in abort
% ---and, therefore, the throughput improvement---
% rate could be significant under certain workloads.




\begin{table}	
\centering
%   \hspace*{-1em}  
\small
  \begin{tabular}{c | c c c c c c c c c | c c c c c}
%   & \multicolumn{6}{c}{\centering Consistency Criteria}
%       \\
%   \cline{2-7}  
  	 							& \multicolumn{9}{c|}{\textbf{CP Models}} & \multicolumn{5}{c}{\textbf{AP Models}} \\
  \emph{\textbf{Anomaly / Model} } & \textbf{SS} & \textbf{S} & \textbf{US} & \textbf{\emph{OP}} & \textbf{\emph{CV}}& \textbf{SI} & \textbf{PSI} & \textbf{\emph{PSI--}} & \textbf{RC}+ & \textbf{TCC} & \textbf{\emph{TCC--}} & \textbf{RA} & \textbf{RC} & \textbf{NI}\\
  											&  &  &  & \textbf{US}  & \textbf{US} & & & &  &  &  &  & &  \\
  \hline
  Dirty Read 								& x & x & x & \textbf{\emph{x}} & \textbf{\emph{x}} & x & x & \textit\textbf{{x}} & x & x & \textit\textbf{{x}} & x & x & -  \\
%   Non-repeatable Reads & x & x & x & x & x & x & x & x & -  \\
  Read Skew 								& x & x & x & \textbf{\emph{-}} & \textbf{\emph{-}} & x & x & \textit\textbf{\textbf{{-}}} & - & x & \textit\textbf{{-}} & x & - & - \\
  Lost Update 								& x & x & x & \textbf{\emph{x}} & \textbf{\emph{x}} & x & x & \textit\textbf{{x}} & x & - & \textit\textbf{{-}} & - & - & - \\
  Write Skew 								& x & x & x & \textbf{\emph{x}} & \textbf{\emph{x}}  & - & - & \textit\textbf{{x}} & - & - & \textit\textbf{{-}} & - & - & -\\ 
  Long Fork			 						& x & x & - & \textbf\emph{{-}} & \textbf\emph{{-}} & x & - & \textit\textbf{{-}} & - & - & \textit\textbf{{-}} & - & - & -\\ 
%   \hline
  Order violation 							& x & x & x & \textbf{\emph{x}} & \textbf{\emph{{-}}} & x & x & \textit\textbf{{x}} & - & x & \textit\textbf{{x}} & - & - & -\\
  Time Violation 							& x & - & - & \textbf\emph{{-}} & \textbf\emph{{-}} & - & - & \textit\textbf{{-}} & - & - & \textit\textbf{{-}} & - & - & -\\

  \end{tabular}
  \caption{Anomaly comparison of new isolation levels}
\label{table:anomalies2}
\end{table}










